The Role of Large Language Models in the Recognition of Territorial Sovereignty: An Analysis of the Construction of Legitimacy

We examine the potential impact of Large Language Models (LLM) on the recognition of territorial sovereignty and its legitimization. We argue that while technology tools, such as Google Maps and Large Language Models (LLM) like OpenAI's ChatGPT, are often perceived as impartial and objective, this perception is flawed, as AI algorithms reflect the biases of their designers or the data they are built on. We also stress the importance of evaluating the actions and decisions of AI and multinational companies that offer them, which play a crucial role in aspects such as legitimizing and establishing ideas in the collective imagination. Our paper highlights the case of three controversial territories: Crimea, West Bank and Transnitria, by comparing the responses of ChatGPT against Wikipedia information and United Nations resolutions. We contend that the emergence of AI-based tools like LLMs is leading to a new scenario in which emerging technology consolidates power and influences our understanding of reality. Therefore, it is crucial to monitor and analyze the role of AI in the construction of legitimacy and the recognition of territorial sovereignty.

==> mysc/CheckList.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} These were highlighted in the Experiments and Conclusion sections.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerNA{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} A link is provided in the Introduction section.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} This is mentioned in the beginning of the Experiments section.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} This is mentioned in the beginning of the Experiments section.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> mysc/oldExperiments.tex <==
\section{Experiments} 
\label{sec:experiments}
In this section, we aim to evaluate the implications of model accuracy and fairness when encoding categorical protected attributes in real datasets for one-hot encoding and target encoding and also compare against the case of not including the protected attribute in the training data. Furthermore, we study the impact of target encoding regularization and extend our experiments towards an inter-sectional fairness case.

In the first experiment, we tackle the fairness implications from the irreducible bias, by comparing two large groups. In the next experiment, we go through the reducible bias case. Finally, in the last experiment, using intersectional fairness, we improve the model performance but also make a more discriminant model for both bias scenarios. We provide empirical evidence of the implications of encoding protected categorical attributes over two datasets: COMPAS and Law School Admission Council.\footnote{Experiments on Law School Admission Council dataset are reported in the appendix (cf. Section~\ref{sec:appendix}).}

\subsection{COMPAS}
\label{sec:experiments.compass}

The scenario we want to address is characterized by datasets that display categorical features with a high cardinality of sensitive attributes in a binary classification problem. We make use of the COMPAS dataset \cite{compass}. COMPAS is an acronym for Correctional Offender Management Profiling for Alternative Sanctions, which is an assistive software and support tool used to predict the risk that a criminal defendant will re-offend. The dataset provides a category-based evaluation labeled as high risk of recidivism, medium risk of recidivism, or low risk of recidivism. We convert this multi-class classification problem into binary classification combining the medium risk and high risk of recidivism vs. low risk of recidivism. The input used for the prediction of recidivism consists of 11 categorical features, including gender, custody status, legal status, assessment reason, agency, language, ethnicity, and marital status. The sensitive feature that we will be looking at is \textit{Ethnic} for the single discrimination, whose protected group will be the most represented group: African-American (cf. Figure~\ref{fig:pieCompas}).


For intersectional fairness, we created the variable \textit{EthnicMarital}, engineered by concatenating \textit{Ethnic} and \textit{Marital} status. This new feature has a high cardinality of 46 distinct values (cf. Figure~\ref{fig:pieCompas}). The most predominant category is \textit{African-American Single}, and it will be the protected group (cf. Figure~\ref{fig:pieCompas}) for the intersectional fairness case. To compare disparate treatment between groups we will make use of  \textit{Caucasian Married} as the reference group. It is worth noting that the contribution of the features to the model performance, based on feature importance explanation mechanism\cite{shapTree,ribeiro2016why,christoph_molnar2019_interpretableML,desiderataECB}, is highly relevant. %In Figure \ref{fig:pieCompas}, the categories of the protected attributes are represented. 
The available data is split into a 50/50 stratified train/test split, maintaining the ratio of each category between train and test set.


\begin{figure}[ht]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.2\linewidth]{images/ethnicPie.eps}
  \caption{\textit{Ethnic} categories distribution}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.2\linewidth]{images/ethnicmaritalPie.eps}
  \caption{Intersectional fairness \textit{EthnicMarital} categories distribution}
\end{subfigure}
\caption{Distribution of the protected attribute categories to be encoded and regularized for the COMPAS data \cite{compass}. %Predominant \textit{Ethnic} categories are \textit{African-American} and \textit{Caucasian}. For the intersectional fairness case (b), the number of categories is increased to 46 distinct groups.
}\label{fig:pieCompas}
\end{figure}

In Figure~\ref{fig:pieCompas}, we show the distributions of the ethnic groups (a) and the intersectional groups of ethnic and marital status (b). There are two groups (\textit{African-American} and \textit{Caucasian}) that account for the $80\%$ of the data, while there are less represented groups such as Asian or Arabic that have a less significant statistical weight. For the intersectional fairness case, the number of groups increases, making room for more distinct, disparate, and imbalanced groups. 



\subsection{Choice of metrics and models}
\label{sec:methodology.metrics}
\subsubsection{Fairness metrics}

We have selected three fairness metrics to showcase the fairness impacts of encoding categorical protected attributes, the three metrics have in common that the lower the value the more fair the model is. 

As we are in high cardinality categorical scenarios ($\sim 10$ distinct values of the protected attribute). We calculate the overall fairness $\mathcal{L}$ of the model $f_\theta$ on data of interest $X$ given a fairness metrics $\ell$, reference group $(j)$ and rest of groups $(i)$ as:
\begin{equation}
    \mathcal{L}(f,X) = \sum_{i \in X\setminus \{j\}} |\ell(\hat{f}(X_j),\hat{f}(X_i)) |
\end{equation}
\begin{itemize}
    \item  \textbf{Equal opportunity fairness.} Following \citet{DBLP:conf/nips/HardtPNS16}'s emphasis on ensuring fair opportunity instead of raw outcomes (it also remains a guiding principle in domains like credit scoring \cite{bigdata_potus,bigdata_potus1}), we choose \emph{equal opportunity} (EO) as a fairness notion and use the metric {\it disparate treatment} (difference between the true positive rates) to measure unfairness, which is estimated using the disparate treatment metric \cite{zafat2017fairnessDisparate}---hence, for simplicity, we refer to the interplay of these concepts as the \textit{equal opportunity fairness (EOF)} metric. The value is the difference in the True Positive Rate (TPR) between the protected group and the reference group: %reference group and the group whose \textit{disparate treatment} we want to evaluate. 
%This metric intuition can be understood as  \emph{equality of opportunity} \cite{hartdt_equality,negligible2021}. We measure TPR disparity as the difference between the recall attained by a model for one group of interest (such as \textit{Caucasian} individuals) and the model’s recall for the reference group \textit{African-American}.

    \begin{equation}\label{eq:TPR}
    \text{TPR} = \frac{\text{TP}}{\text{TP + FN}} \hspace{2cm} \text{Equal Opportunity Fairness} = \text{TPR}_j - \text{TPR}_i
    \end{equation}

    A negative value in (\ref{eq:TPR}) is due to the worse ability of a Machine Learning model to find actual recidivists for the protected group (i) in comparison with the reference group (j).

    
    \item Statistical Parity (Strong Demographic Parity): The difference between favourable out-comes received by the unprivileged group and privileged group ~\cite{kamishima2012fairness,DBLP:conf/icml/ZemelWSPD13,DBLP:conf/kdd/FeldmanFMSV15,DBLP:conf/kdd/Corbett-DaviesP17}. SDP ensures that a fair decision does not depend on the sensitive attribute regardless of the classification threshold used  \cite{DBLP:conf/uai/JiangPSJC19,DBLP:conf/aaai/ChiappaJSPJA20} $d(P(f_\theta(X)|Z=i),P(f_\theta(X)|Z=j))=0$ where $d(\cdot,\cdot)$ is a distance function. In this work we use the Wasserstein distance as a measure between the two probabilistic distributions.
    
    \item Average Absolute Odds (Equalized Odds): The sum of the absolute differences between the True Positive Rates and the False Positive Rates of the unprivileged group plus the same ratio for the  privileged group.
    
    \begin{equation}\label{eq:AAO}
    \text{FPR} = \frac{\text{FP}}{\text{FP + TN}} \hspace{2cm} \text{Average Absolute Odds} = |TPR_j - FPR_j| + |TPR_i - FPR_i|
    \end{equation}

\end{itemize}
\subsubsection{Model performance} For model performance metrics, as we are in a binary classification scenario, we use the Area Under the Curve (AUC)---a  metric that illustrates the diagnostic ability of a binary classifier system as its discrimination threshold is varied \cite{statisticallearning}. This metric is less susceptible to class imbalance than accuracy or precision and also accepts soft probabilities predictions. % is an adequate candidate for our problem. For less technical readers is worth noting that 
An AUC of 0.5 is equal to doing random predictions, which can be used as a baseline for interpreting the model performance results. Previous work on fair machine learning experiments on COMPAS have focused on using accuracy as a performance metric \cite{zafat2017fairnessDisparate,zafar2017parity,zafar2017fairness}, but given the target ratio of the full dataset of COMPAS $(70:30)$, we consider accuracy to be a less informative measure of model performance. 

\subsubsection{Machine learning algorithms} As classification estimators, we experiment with a linear regression model, a decision tree model, and a gradient boosting decision tree. All models are trained on the training set. These three models provide examples of a model with large bias (the linear regression model), a model with large variance (the decision tree model), and an extensively used and with state-of-the-art performance model (gradient boosting decision tree) \cite{supervised_learning_algorithms,gbm_travel,gbm,gbm_nn,get_bristol}.


\subsection{Irreducible bias}
\label{exp:first}

The irreducible bias that is induced while encoding categorical features is due to different posterior probabilities among groups. It can be observed for large groups, where instead reducible bias due to variance is low. For this case, we will choose the two largest groups in the COMPAS dataset: \textit{African-American} and \textit{Caucasian}, (Figure~\ref{fig:pieCompas}). Recall that we will benchmark the trade-off between disparate treatment and AUC metrics while using two different encoding techniques (Section~\ref{sec:relatedwork}), with two different regularization techniques (Section~\ref{sec:methodology}) and three different estimators (Section~\ref{sec:methodology.metrics}). 

The ranges of the regularization hyperparameters are:  $\lambda \in$ $[0,1]$ for the width of the Gaussian noise regularization;  $m \in [0,10000]$ for the additive smoothing using the $m$-probability estimate function $\lambda(n_i) = n_i/(n_i+m)$ (see \cite{high-cardinality-categorical}). These hyperparameters will also be kept for the rest of the experiments for this dataset. 
The observed group target mean, namely $\hat{p}_i = n_{i, Y}/n_i$, is  $0.43$ for \textit{African-American}, and $0.25$ for \textit{Caucasian}.
%\sr{This statement does not make sense in English.}

\begin{figure}[ht]
    \centering
    \includegraphics[width=1.1\linewidth]{images/encCompassFull.eps}
    \caption{Comparing one-hot encoding and target encoding regularization (Gaussian noise and smoothing) for the Logistic Regression, Decision Tree, and Gradient Boosting classifiers over the test set of the COMPAS dataset. The protected group is \textit{African-American}. Reference group is \textit{Caucasian}. Red dots regard different regularization parameters: the darker the red the higher the regularization. Blue dot regards the one-hot encoding.}
    \label{fig:compas1}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/compassHyperGaussian.eps}
    \caption{Impact of the Gaussian noise regularization parameter $\lambda$ on performance and fairness metrics over the test set of the COMPAS dataset. In the left image the AUC of the protected group, reference group, and global over the regularization hyperparameter. On the right, the equal opportunity fairness variation throughout the regularization hyperparameter.
    %\sr{Remove TPR from the y-axis label} \sr{what classification model does this figure refer to?}  \sr{Describe what are the 'tot', 'African-American' and 'Caucasian' lines on the left plot. Not said/discussed in the text!} \sr{put space between the left and right plots}
    }
    \label{fig:hyperCompas}
\end{figure}

Figure \ref{fig:compas1} shows that the smoothing regularization effects are relevant for the logistic regression and negligible in both fairness and model performance for the other estimators. On the other hand, Gaussian regularization affects both metrics for all estimators. This is due to the adding of white noise to the data inhibiting learning. From Figure \ref{fig:hyperCompas}, we can see that there is an optimal value around $0.3$, where the disparate treatment has become negligible and the model performance has only slightly decreased. It is worth noting that performances for both groups have a negative slope. For the one-hot encoding (blue dot), the performance is very similar to the best target encoding (in terms of AUC). But, when the target encoder is correctly regularized (red dots) it achieves less or equal discriminant results consistently. 

\subsection{Reducible bias}
\label{exp:secondorder}

This second type of bias arises due to the large variance found when sampling small groups. To replicate this biased situation, from the most common ethnic group, \textit{African-American}, we sample a $\approx 0.002$ fraction, being the ratio of $50$ against $27,000$ samples (cf. Figure \ref{fig:pieCompas}). We treat this sampled group as it were a different category than the original \textit{African-American} group. Both come from the same distribution so if we had enough statistical mass for both of them, the encoding should be the same. We note that due to the stochastic nature of this sampling experiment, different randomization seeds will produce different results. For this split, the mean of the sampled group is $0.63$ while the reference group has a mean of $0.43$. The regularization hyperparameters are the same as in the previous experiment (Section~\ref{exp:first}).

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/encTheory.eps}
        
    \caption{One-hot Encoding vs regularized target encoding (Gaussian and smoothing), comparing the reference group \textit{African-American} over a sample of the reference group. Smoothing regularization reduces group equal opportunity fairness with a negligible loss of AUC.
    Red dots regard different regularization parameters: the darker the red the higher the regularization. Blue dot regards one-hot encoding. Over tuning Gaussian noise hyperparameter causes a noticeable drop in performance. 
    %\sr{Rewrite caption as for / consistently with Figure 2}
    }
    \label{fig:theory}
\end{figure}


In Figure \ref{fig:theory}, we can see a logistic regression estimator that is fed encoded variables in the two different encoding ways. Non-regularized target encoding is more discriminant than one-hot encoding and the AUC is almost the same with negligible differences. For the smoothing regularization, it is curious to see that the model performance does not vary, but the fairness does so significantly. This is due to the regularization affecting only to categories with few samples and the global AUC being almost unaffected. For the Gaussian noise regularization, the effect is quite similar to the smoothing, but in case the $\lambda$ hyperparameter is over-tuned, the model performance drops significantly.
%Does smoothing effect only for categories with small data and Gaussian irrelevant of the data size? -- YES. Gaussian Encoder regularizes independent of the statistical mass of the minority category. While smoothing only for categories with few samples.

%Smoothing has a low impact on accuracy, while Gaussian has a progressive impact.



\subsection{Intersectional Fairness}
\label{exp:intersectional}

A common feature engineering technique that boosts model performance consists of concatenating two or more categorical features \cite{howtowinKaggle}. If the categorical features are protected attributes, the fairness problem is known as intersectional fairness \cite{RomeiR2014_DiscSurvey, Wachter2021_FairnessCantAutomate} (Section~\ref{sec:relatedwork.intersectional}). To provide evidence of the potential effects of encodings on intersectional fairness, we concatenate \textit{Ethnic} and \textit{Marital} status of the COMPAS dataset.  We select \textit{African-American Single} as the protected group and \textit{Caucasian Married} as the reference group. Both groups have enough statistical mass so the induced bias is not due to variance but rather it is irreducible bias. The group target mean is $0.46$ for \textit{African-American Single} and $0.10$ for \textit{Caucasian Married}. This is an increased difference between the two groups with respect to previous experiments when comparing single groups of \textit{African-American} and \textit{Caucasian}. 
 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/interCompasLinear.eps}
    \caption{Intersectional fairness case. One-hot Encoding vs regularized target encoding (Gaussian and smoothing), comparing \textit{African American Single} and \textit{Caucasian Married}.}
    \label{fig:regularization_inter}
\end{figure}

In Figure \ref{fig:regularization_inter}, we can see how feature concatenation can slightly boost the model performance to an AUC of $0.713$ using one-hot encoding against $0.709$ for the single group case (Figure~\ref{fig:compas1}). But we can also see how it worsen fairness: one-hot encoding achieves $-0.21$ of equal opportunity fairness (Figure~\ref{fig:compas1}) under single features, and $-0.28$ when using concatenated features. The Gaussian regularization overperforms smoothing in terms of fairness and model accuracy, not only the maximum values achieved but also at intermediate stages of regularization. This is not surprising, and, in general, feature concatenation can worsen fairness both on the side of irreducible bias (because $p_i$ and $p_r$ become more distant) and on the side of reducible bias (because $n_i$ becomes smaller).
